ConnectIt: A Framework for Static and Incremental Parallel Graph Connectivity Algorithms

Connected components is a fundamental kernel in graph applications. The fastest existing parallel multicore algorithms for connectivity are based on some form of edge sampling and/or linking and compressing trees. However, many combinations of these design choices have been left unexplored. In this paper, we design the ConnectIt framework, which provides different sampling strategies as well as various tree linking and compression schemes. ConnectIt enables us to obtain several hundred new variants of connectivity algorithms, most of which extend to computing spanning forest. In addition to static graphs, we also extend ConnectIt to support mixes of insertions and connectivity queries in the concurrent setting. We present an experimental evaluation of ConnectIt on a 72-core machine, which we believe is the most comprehensive evaluation of parallel connectivity algorithms to date. Compared to a collection of state-of-the-art static multicore algorithms, we obtain an average speedup of 12.4x (2.36x average speedup over the fastest existing implementation for each graph). Using ConnectIt, we are able to compute connectivity on the largest publicly-available graph (with over 3.5 billion vertices and 128 billion edges) in under 10 seconds using a 72-core machine, providing a 3.1x speedup over the fastest existing connectivity result for this graph, in any computational setting. For our incremental algorithms, we show that our algorithms can ingest graph updates at up to several billion edges per second. To guide the user in selecting the best variants in ConnectIt for different situations, we provide a detailed analysis of the different strategies. Finally, we show how the techniques in ConnectIt can be used to speed up two important graph applications: approximate minimum spanning forest and SCAN clustering.

==> inputs/code_sample.tex <==
\definecolor{light-gray}{gray}{0.95}
\definecolor{dark-gray}{gray}{0.25}

\begin{figure}[t]
\begin{minted}[fontsize=\small,linenos=true,numbers=left,autogobble,numbersep=2pt,xleftmargin=0.5em,escapeinside=||]{cpp}
#include "connectit.h"|\label{line:importconn}|
sequence<uint64_t> DensityCluster(Pointset& P) {
  auto graph = BuildDensityGraph(P);|\label{line:density}|
  auto labeling = connectit::union_find_alg<|\label{line:connectitstart}|
   /* sampling method = */  sample_ldd,
   /* union method = */     union_rem_cas,
   /* path compression = */ find_compress,
   /* splice rule = */      atomic_halve>(graph); |\label{line:connectitend}|
  return labeling;
}
\end{minted}
\caption{Sample \framework{} code for instantiating the \framework{}
framework in the context of a density-clustering algorithm. The
algorithm first constructs a graph using a density-based method, such
as DBSCAN (Line~\ref{line:density}). The second step applies a
\framework{} union-find algorithm using a specified sampling method,
union method, path compression rule, and splice rule. This step
returns a mapping from vertices (points) to connectivity labels, which
is returned as the output clustering. Similar code can be used to
invoke any of the other algorithms that can be generated by
\framework{}.
}
\label{fig:codesample}
\end{figure}


==> inputs/framework_case_study.tex <==
\subsection{\framework{} Case Study}\label{sec:case_study}

In this section we present a case-study of our fastest \framework{}
algorithm combined under different sampling strategies for the
symmetrized Twitter graph dataset, and discuss how our approach yields
much higher performance than existing state-of-the-art approaches. We
discuss how our \unionremcas{} algorithm using the \splitone{} splice
rule, with no additional compression compares with (i) a
state-of-the-art theoretically efficient connectivity algorithm, based
on recursively applying low-diameter
decomposition~\cite{SDB14} (ii) the Afforest algorithm,
which is the current state-of-the-art approach for multicore
connectivity, and (iii) our algorithm applied without sampling.

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.95\columnwidth]{figs/case_study_running_time}
\caption{\label{fig:case_study_running_time}
}
\end{center}
\end{figure}

Figure~\ref{fig:case_study_running_time} shows the running times for
our code under each sampling scheme, the running time of each sampling
scheme individually, as well as the three comparisons listed above.
%
The sampling scheme constitutes the majority of the overall cost.
94\% of the running time for BFS
95.7\% of the running time for $k$-Out.
95.9\% of the running time for LDD.
%
Without sampling, we are 1.83x slower than Afforest, but still 1.85x
faster than WorkefficientCC.
Thus, sampling is critical for achieving state-of-the-art performance.
%

Discuss sampling time for Afforest, and some explanations for why we
are faster.

Discuss edges examined for WorkefficientCC, and the number of edges we
examine.





==> inputs/long_overview.tex <==
\subsection*{\framework Overview}

The \framework{} framework is designed for \emph{\minbased{}
connectivity algorithms}, which are based on vertices propagating
labels to other vertices that they are connected to, and updating
labels based on the minimum received label. All of the algorithms
conceptually view the label of a vertex $v$ as a directed edge from
$v$ to the vertex corresponding to $v$'s label. Thus, these directed
edges form a set of directed trees. All of the algorithms we study
maintain acyclicity in this forest (ignoring self-loops at the roots
of trees). The \minbased{} algorithms that we study in this paper
include both \emph{root-based algorithms} which include a broad class
of union-find algorithms and several other algorithms, which only
modify the labels of roots of trees in the forest, as well as
\emph{\otherminbased{} algorithms} which deviate from this rule and can
modify the labels of non-root vertices.


\myparagraph{Union-Find} Union-find algorithms for connectivity
maintain vertices in disjoint sets, represented as rooted trees. Sets
are combined based on membership of the endpoints of each edge by
changing the parent pointer of the root of one tree to point to a
vertex in another tree. At termination, the disjoint sets define the
\components{} of the graph. \framework{} includes different
concurrent union-find algorithms, obtained by using different rules
for uniting two sets and for path compression during find operations.
The rules for union are based on concurrent versions of Rem's
algorithm~\cite{Patwary2012}, randomized linking by
ID~\cite{Jayanti2016}, and randomized linking by
rank~\cite{JayantiTB19}. The path compression techniques include
path-halving, path-splitting, full path compression, and splicing.

The concurrent randomized linking by ID and randomized linking by rank
algorithms were proposed and analyzed theoretically by Jayanti et
al.~\cite{Jayanti2016,JayantiTB19}.
A variant of one of these algorithms using
path-halving was recently implemented on GPUs by Jaiganesh and
Burtscher~\cite{Jaiganesh2018}.
\framework incorporates all of the implementation choices in the
algorithms by Jayanti et al. We also introduce the full path
compression technique, which we found to work better in practice in
some cases. Patwary et al.~\cite{Patwary2012} present two multicore
implementations of Rem's algorithm with splicing, one which is a
natural extension of the serial algorithm to use locks, and the other
is a lock-free implementation using speculative execution (we found their
lock-free implementation to not always produce the correct result).
\framework includes the lock-based Rem's algorithm by Patwary et
al.~\cite{Patwary2012}, but also introduces a lock-free version using
compare-and-swap.
In addition to splicing, \framework also supports
path-halving and path-splitting for path compression in Rem's
algorithm. We prove that our multicore implementations of Rem's
algorithm are \emph{phase-concurrent}~\cite{ShunB14} in that the
algorithm produces correct results as long concurrent operations at
any time only consist of either only unions or only finds.  Blelloch
et al.~\cite{BFGS12} present a deterministic multicore union-find connectivity
algorithm based on linking by ID that is also phase-concurrent.

Very recently, Alistarh et al.~\cite{alistarh2019search} performed a
performance evaluation of concurrent union-find implementations for
multicores on much smaller graphs. They introduce a lock-free version
of concurrent Rem's algorithm with path-splitting similar to our
implementation, but do not prove that the algorithm is correct, or
consider other path-compaction methods in their algorithm.
\framework{} implements a similar lock-free Rem's algorithm that is
more general, allowing the algorithm to be combined with path-halving,
and splicing in addition to path-splitting.

Using \framework, we can obtain a total of 144 different concurrent
union-find implementations. Our union-find
algorithms can be used both for \components{} and for spanning
forest, and support incremental updates to the graph.  Similar in
spirit to the experimental analysis of 55 different sequential
union-find implementations by Patwary et al.~\cite{Patwary10}, we
analyze the performance of our 144 union-find implementations in the
parallel setting.

\myparagraph{Other Root-Based Algorithms}
As discussed earlier, we classify the union-find algorithms above in
our framework as \emph{root-based algorithms}, in that each of their
union operations only performs a link if it operates on the root of a
tree.  Other than union-find, another classic parallel \components{}
algorithm that falls under this categorization is the Shiloach-Vishkin
(SV) algorithm, which \framework{} includes.  Many variants of SV have
been described in the
  literature~\cite{Awerbuch1987,Cong2014,Bader2005a,Greiner94,BeamerAP15,Soman,Meng2019,Wang2017,Pai2016,Ben-Nun2017,Zhang19fastsv},
but none of these implementations combine SV with sampling approaches,
as done in this paper.

\myparagraph{Other Min-Based Algorithms}
The other class of \minbased{} algorithms that we study work as follows.
These algorithms scan all edges and for each edge, apply an operation
that modifies the parents of the endpoints over a number of rounds. On
each round, the algorithm tries to update the parents of vertices
based on the values of their current parents, updating a parent only
if the new parent is \emph{smaller} than the previous one, hence the
name for this category. The algorithm terminates once the parent
values stop changing. One example of such an algorithm is the folklore
label-propagation algorithm.

In \framework{}, we implement a recent \minbased{} algorithm by Stergiou
et al.~\cite{Stergiou2018}, as well as 16 algorithms from a framework
described recently by Liu and Tarjan~\cite{LiuT19}, but were not
implemented. To the best of our knowledge, these are the first
implementations and experimental evaluation of the algorithms by Liu
and Tarjan.  Stergiou et al.~\cite{Stergiou2018} provide a
distributed-memory implementation of their algorithm, which we adapt
to the multicore setting. A subset of the Liu-Tarjan algorithms
perform updates only to roots of trees, and thus can also be
categorized as root-based algorithms.

\myparagraph{Sampling and Two-phase Execution} Inspired by the
Afforest algorithm~\cite{Sutton2018}, \framework produces algorithms
with two phases: the \defn{sampling} phase and the \defn{finish}
phase. In the sampling phase, we run \components{} on a subset of the
edges in the graph, which assigns a temporary label to each vertex. We
then find the most frequent label, $L_{\max}$, which corresponds to the
ID of the largest component (not necessarily maximal) found so far.
In the finish phase, we only need to run \components{} on the incident
edges of vertices with a label not equal to $L_{\max}$, which can
significantly reduce the number of edge traversals. We observe that
this optimization is similar in spirit to the direction-optimization
in breadth-first search~\cite{Beamer12}, which skips over incoming
edges for vertices, once they have already been visited during dense
iterations. If sampling is not used, then the finish phase is
equivalent to running one of the previously described algorithms on
all vertices and edges.

The sampling strategy of the Afforest algorithm~\cite{Sutton2018} runs
connectivity on the first $k$ edges out of each vertex using a variant
of union-find, and then uses the same union-find algorithm for the
finish phase.  \framework implements a sampling strategy similar to
Afforest, but instead of picking the first $k$ edges out of each
vertex, we pick the first edge out of every vertex, and $k-1$ random
edges out of each vertex to avoid adversarial inputs.  We then use any
of our 144 union-find variants on these edges. We refer to
this strategy as \defn{$\textbf{k}$-out}.
\framework includes another sampling strategy, which is to run
direction-optimizing breadth-first search from a random sample of
vertices, such that the largest connected component is likely to be
explored.  $L_{\max}$ is set to be the label of vertices in the largest
component found.  Lastly, we include a sampling strategy based on
computing a low-diameter decomposition
(LDD)~\cite{MillerPX2013,DhBlSh18,SDB14} of the graph, which
partitions the graph into connected sets of vertices, such that the
diameter of each set is small and the number of edges between sets is
small. $L_{\max}$ is then set to be the label of vertices in the
largest set in the decomposition.

Our main observation is that these sampling techniques are general
strategies that reduce the number of edge traversals in the finish
phase, and thus accelerate the overall algorithm.
In \framework, any of the \minbased{} algorithms we consider can be used
for the finish phase in combination with any of the three sampling
schemes.  For the implementations where the finish phase is a
root-based algorithm, \framework also supports spanning forest
computation.  Our generalized sampling paradigm and integration into
\framework enables us to express over 232 combinations of parallel
algorithms of parallel graph connectivity and 192 implementations for
parallel spanning forest (note that only our root-based algorithms are
supported for spanning forest).


\myparagraph{Incremental Connectivity} Due to the frequency of updates
to graphs, various parallel streaming algorithms for connected
components have been
developed~\cite{McColl13,Ediger12,Simsiri2017,Sengupta17,Acar2019,dhulipala2020parallel}.
Motivated by this, the \framework framework supports a combination of
edge insertions and connectivity queries in the graph.  Both the
union-find and root-based algorithm implementations in \framework
support batched edge insertions/queries.  Additionally, all of the
union-find implementations other than Rem's algorithms combined with
the splice compression scheme support asynchronous updates and
queries, and most of them are lock-free or wait-free.

\myparagraph{Experimental Evaluation} The \framework framework enables
one to easily combine different algorithmic choices into a single
program to achieve high performance for parallel connectivity and
spanning forest. We conduct a comprehensive experimental evaluation of
all of the connectivity implementations in \framework on a 72-core
multicore machine, in both the static and incremental setting.  Using
hardware performance counters, we analyze the tradeoffs of different
strategies in terms of their work and locality. The trends for the
spanning forest implementations are similar to connectivity, and on
average the additional overhead needed to obtain the spanning forest
compared to connectivity is 23.7\%.

\input{inputs/big_comparison}

Compared to existing work, \framework implementations significantly
outperform state-of-the-art implementations using the new sampling
techniques proposed in this paper, and often outperform prior work
even without applying sampling. Our fastest algorithms using sampling
are always faster than the fastest currently available implementation.
As an example of our performance, \framework is able to produce
implementations that can process the Hyperlink2012
graph~\cite{meusel15hyperlink}, which is the largest publicly-available
real-world graph and has over 3.5 billion vertices and 128 billion
edges, on a single 72-core machine with a terabyte of RAM. We show
existing results on this graph, and the smaller Hyperlink2014 graph
(1.7 billion vertices and 64 billion edges) in
Table~\ref{table:big_comparison}. Our running times are between
3.65--41.5x faster than existing distributed-memory results that
report results for Hyperlink2012, while using orders of magnitude
fewer computing resources. \framework also significantly outperforms
existing state-of-the-art multicore connectivity algorithms for this
graph, improving on the previous fastest algorithm from
GBBS~\cite{DhBlSh18} by over 3.14x on the same machine.


==> inputs/sampling_graph_table.tex <==



==> inputs/streaming_cpu_fastest_updates_only.tex <==
\begin{table*}[!t]
\footnotesize
\centering
\vspace{-3em}
\hspace*{-1.5em}
\begin{tabular}[t]{  l | c | c | c | c | c | c | c | c | c | c}
  \toprule
  {\bf Algorithm} &  \multicolumn{1}{c|}{\bf RO} & \multicolumn{1}{c|}{\bf LJ} & \multicolumn{1}{c|}{\bf CO} & \multicolumn{1}{c|}{\bf TW}  & \multicolumn{1}{c}{\bf FR} & \multicolumn{1}{c|}{\bf RMAT} & \multicolumn{1}{c}{\bf BA} & \multicolumn{1}{c}{\bf CW} & \multicolumn{1}{c}{\bf HL14} & \multicolumn{1}{c}{\bf HL12} \\
  \midrule
  \unionearly{}         &1.48e9  &9.23e8  & 1.38e9 & 4.31e8 & 1.05e9 &3.49e8 &5.16e8   &4.00e8   &3.15e9   &2.80e9  \\
  \unionhook{}          &3.12e9  &4.21e9  & 5.94e9 & 2.79e9 & 1.49e9 &7.27e8 &1.18e9   &4.69e9   &5.17e9   &4.48e9  \\
  \unionasync{}         &3.49e9  &3.36e9  & 5.29e9 & 2.73e9 & 1.41e9 &8.05e8 &1.13e9   &4.86e9   &5.92e9   &4.69e9  \\
  \unionremcas{}        &{\bf \color{mygreen}3.98e9}  &{\bf \color{mygreen}5.28e9}  &{\bf \color{mygreen}7.16e9} &{\bf \color{mygreen} 3.85e9} & {\bf \color{mygreen}2.01e9} &{\bf \color{mygreen}8.78e8} &{\bf \color{mygreen}1.46e9}&{\bf \color{mygreen}5.73e9}   &{\bf \color{mygreen}6.64e9}   &{\bf \color{mygreen}5.64e9}  \\
  \unionremlock{}       &1.56e9  &3.68e9  & 5.95e9 & 3.36e9 & 1.74e9 &7.67e8 &1.42e9  &3.56e9   &2.99e9   &3.21e9 \\
  \jayanti{}            &1.15e9  &1.06e9  & 2.68e9 & 1.42e9 & 7.33e8 &2.88e8 &5.27e8  &2.15e9   &2.26e9   &1.79e9 \\
  \liutarjan{}          &2.87e8  &4.31e8  & 5.98e8 & 3.77e8 & 1.84e8 &1.11e8 &1.98e8  &3.02e8   &2.80e8   &2.62e8 \\
  \shiloachvishkin{}    &1.79e8  &4.56e8  & 1.13e9 & 2.89e8 & 1.76e8 &1.06e8, &2.43e8 &3.34e8   &2.65e8   &2.24e8  \\
\end{tabular}
\caption{\small Maximum parallel streaming throughput (directed edge updates
  per second) achieved by \framework{} streaming algorithms on our
  graph inputs, and two synthetic graph inputs from the RMAT and
  Barabasi-Albert (BA) families.  Due to memory constraints, we were
  unable to materialize a COO representation of our three largest
  graphs, and instead, sample of 10\% of the edges for the batch.
  Otherwise, the entire graph is used as part of a single batch, which
  is not permuted.  All edges in the batch are updates. For each graph
  we display the algorithm with the highest throughput in bold.}
\label{table:streaming_cpu_all}
\end{table*}

